Sensitivity and environmental response of the CMS RPC gas gain monitoring system

Results from the gas gain monitoring (GGM) system for the muon detector using RPC in the CMS experiment at the LHC is presented. The system is designed to provide fast and accurate determination of any shift in the working point of the chambers due to gas mixture changes.

==> lnfprepCMS.tex <==
% This style file will produce a LaTeX article formatted as requested
% by Frascati Physics Series published by 
% S.I.S.-Laboratori Nazionali di Frascati. It is basically
% the standard art12.sty, with modifications as needed.
% Usage: begin your document with
%  \documentstyle[frascatiphys]{article}
% See also frascatiphys.tex.
%
% The user MUST use \author{} to contain both authors' names and 
%       institutions; use \\ to separate lines.
%       all caps for title, roman for author names, and italic (\em)
%       for institution names and addresses.
%       Only 10 cm are allowed for your title and
%       author.  For large collaborations, you may need to
%       list individual names in a footnote.
% History:
% Nov-1-89      T. Nguyen       added \pagestyle{empty} at the end
%                               and modified \maketitle command to 
%                               use pagestyle empty instead of plain.
% Sep-1-94      S. Bianco LNF   Make this style compatible with
%                               Frascati Physics Series format.
% Sep-29-96     SB              include semiheader in titlepage
% Feb-17-97     SB LI           indent to 1.00cm, Abstract in bold.
% Set-97        GI              Citations and footskip modified

\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox   
       to 0pt{$^{\@thefnmark}$\hss}}   
   \if@twocolumn               
     \twocolumn[\@maketitle]   
     \else \newpage
     \global\@topnum\z@        % Prevents figures from going at top of page.
     \@maketitle \fi\thispagestyle{empty}\@thanks 
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 \gdef\@thanks{}\gdef\@author{}\gdef\@title{}\let\thanks\relax}

\def\@maketitle{\newpage
 \null
 \vbox to 15cm{                 %space limit for title/author
 \vskip 1em                    % Vertical space above title.
 \begin{center}
  {\scriptsize\bf \@title \par}     % Title set in \normalsize. 
  \vskip 0.5em                % Vertical space after title.
  {\normalsize                % each author set in \normalsize,\bf in a
   \lineskip .5em             % tabular environment
   \begin{tabular}[t]{c}\@author 
   \end{tabular}\par}                   
  \vskip 1em              % Vertical space after author.
\end{center}
 \par
 \vskip 0.5em}                % Vertical space after title/author lines
 }                      % end of vbox to 10cm
\def\abstract{\if@twocolumn
\section*{Abstract}
\else \normalsize
\begin{center}
{ \vspace{-1.0em} {\bf Abstract} \vspace{-.5em}\vspace{0pt}} 
\end{center}
%\quotation 
\fi}
\def\endabstract{\if@twocolumn\else \par\noindent \fi}

% Collapse citation numbers to ranges.  
\newcount\@tempcntc
\def\@citex[#1]#2{\if@filesw\immediate\write\@auxout{\string\citation{#2}}\fi
  \@tempcnta\z@\@tempcntb\m@ne\def\@citea{}\@cite{\@for\@citeb:=#2\do
    {\@ifundefined
       {b@\@citeb}{\@citeo\@tempcntb\m@ne\@citea
        \def\@citea{,\penalty\@m\ }{\bf ?}\@warning
       {Citation `\@citeb' on page \thepage \space undefined}}%
    {\setbox\z@\hbox{\global\@tempcntc0\csname b@\@citeb\endcsname\relax}%
     \ifnum\@tempcntc=\z@ \@citeo\@tempcntb\m@ne
       \@citea\def\@citea{,\penalty\@m}
       \hbox{\csname b@\@citeb\endcsname}%
     \else
      \advance\@tempcntb\@ne
      \ifnum\@tempcntb=\@tempcntc
      \else\advance\@tempcntb\m@ne\@citeo
      \@tempcnta\@tempcntc\@tempcntb\@tempcntc\fi\fi}}\@citeo}{#1}}
\def\@citeo{\ifnum\@tempcnta>\@tempcntb\else\@citea
  \def\@citea{,\penalty\@m}%
  \ifnum\@tempcnta=\@tempcntb\the\@tempcnta\else
   {\advance\@tempcnta\@ne\ifnum\@tempcnta=\@tempcntb \else
\def\@citea{--}\fi
    \advance\@tempcnta\m@ne\the\@tempcnta\@citea\the\@tempcntb}\fi\fi}


%*** below here, standard LaTeX art12.sty with modifications indicated

% art12.sty 23 Sep 85
\lineskip 1pt \normallineskip 1pt
\def\baselinestretch{1}

\def\@normalsize{\@setsize\normalsize{15pt}\xiipt\@xiipt
\abovedisplayskip 12pt plus3pt minus7pt\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip \z@ plus3pt\belowdisplayshortskip 6.5pt plus3.5pt
minus3pt}
\def\small{\@setsize\small{13.6pt}\xipt\@xipt
\abovedisplayskip 11pt plus3pt minus6pt\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip \z@ plus3pt\belowdisplayshortskip 6.5pt plus3.5pt
minus3pt
\def\@listi{\parsep 4.5pt plus 2pt minus 1pt
 \itemsep \parsep
 \topsep 9pt plus 3pt minus 5pt}}
\def\footnotesize{\@setsize\footnotesize{12pt}\xpt\@xpt
\abovedisplayskip 10pt plus2pt minus5pt\belowdisplayskip \abovedisplayskip
\abovedisplayshortskip \z@ plus3pt\belowdisplayshortskip 6pt plus3pt minus3pt
\def\@listi{\topsep 6pt plus 2pt minus 2pt\parsep 3pt plus 2pt minus 1pt
\itemsep \parsep}}
\def\tiny{\@setsize\tiny{7pt}\vipt\@vipt}
\def\scriptsize{\@setsize\scriptsize{9.5pt}\viiipt\@viiipt}
\def\large{\@setsize\large{18pt}\xivpt\@xivpt}
\def\Large{\@setsize\Large{22pt}\xviipt\@xviipt}
\def\LARGE{\@setsize\LARGE{25pt}\xxpt\@xxpt}
\def\huge{\@setsize\huge{30pt}\xxvpt\@xxvpt}
\let\Huge=\huge
\normalsize 
\if@twoside \oddsidemargin 21pt \evensidemargin 59pt \marginparwidth 85pt
\else \oddsidemargin 0.46cm \evensidemargin 0.46cm
 \marginparwidth 68pt 
\fi
\marginparsep 10pt 
\topmargin 0.81cm \headheight 0pt \headsep 0pt \footheight 0pt 
\footskip 35pt 

%*** changed text sizes
\textheight 22cm \textwidth 15cm \columnsep 10pt \columnseprule 0pt 

\footnotesep 8.4pt 
\skip\footins 10.8pt plus 4pt minus 2pt 
\floatsep 14pt plus 2pt minus 4pt \textfloatsep 20pt plus 2pt minus 4pt
\intextsep 14pt plus 4pt minus 4pt \@maxsep 20pt \dblfloatsep 14pt plus 2pt
minus 4pt \dbltextfloatsep 20pt plus 2pt minus 4pt \@dblmaxsep 20pt 
\@fptop 0pt plus 1fil \@fpsep 10pt plus 2fil \@fpbot 0pt plus 1fil 
\@dblfptop 0pt plus 1fil \@dblfpsep 10pt plus 2fil \@dblfpbot 0pt plus 1fil
\marginparpush 7pt 

%***change indents to 1.00cm

\parskip 0pt plus 1pt \parindent 1.00cm  \topsep 10pt plus 4pt minus 6pt
\partopsep 3pt plus 2pt minus 2pt \itemsep 5pt plus 2.5pt minus 1pt 
\@lowpenalty 51 \@medpenalty 151 \@highpenalty 301 
\@beginparpenalty -\@lowpenalty \@endparpenalty -\@lowpenalty \@itempenalty
-\@lowpenalty 
\def\part{\par \addvspace{4ex} \@afterindentfalse \secdef\@part\@spart} 
\def\@part[#1]#2{\ifnum \c@secnumdepth >\m@ne \refstepcounter{part}
\addcontentsline{toc}{part}{\thepart \hspace{1em}#1}\else
\addcontentsline{toc}{part}{#1}\fi { \parindent 0pt \raggedright 
 \ifnum \c@secnumdepth >\m@ne \normalsize\bf Part \thepart \par\nobreak \fi 
\normalsize\bf #2\markboth{}{}\par } \nobreak \vskip 3ex \@afterheading } 
\def\@spart#1{{\parindent 0pt \raggedright 
 \normalsize \bf 
 #1\par} \nobreak \vskip 3ex \@afterheading } 
\def\section{\@startsection {section}{1}{\z@}{-3.5ex plus -1ex minus 
 -.2ex}{2.3ex plus .2ex}{\normalsize\bf}} 
\def\subsection{\@startsection{subsection}{2}{\z@}{-3.25ex plus -1ex minus 
 -.2ex}{1.5ex plus .2ex}{\normalsize\bf}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-3.25ex plus
 -1ex minus -.2ex}{1.5ex plus .2ex}{\normalsize\sl}}
%\def\paragraph{\@startsection *** not defined for this style sheet
%\def\subparagraph{\@startsection *** not defined for this style sheet

%*** remainder left as is

\setcounter{secnumdepth}{3}

\def\appendix{\par
 \setcounter{section}{0}
 \setcounter{subsection}{0}
 \def\thesection{\Alph{section}}}


\leftmargini 2.5em
\leftmarginii 2.2em \leftmarginiii 1.87em \leftmarginiv 1.7em \leftmarginv 1em
\leftmarginvi 1em
\leftmargin\leftmargini
\labelwidth\leftmargini\advance\labelwidth-\labelsep
\labelsep .5em
\parsep 5pt plus 2.5pt minus 1pt
\def\@listi{\leftmargin\leftmargini}
\def\@listii{\leftmargin\leftmarginii
 \labelwidth\leftmarginii\advance\labelwidth-\labelsep
 \topsep 5pt plus 2.5pt minus 1pt
 \parsep 2.5pt plus 1pt minus 1pt
 \itemsep \parsep}
\def\@listiii{\leftmargin\leftmarginiii
 \labelwidth\leftmarginiii\advance\labelwidth-\labelsep
 \topsep 2.5pt plus 1pt minus 1pt 
 \parsep \z@ \partopsep 1pt plus 0pt minus 1pt
 \itemsep \topsep}
\def\@listiv{\leftmargin\leftmarginiv
 \labelwidth\leftmarginiv\advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
 \labelwidth\leftmarginv\advance\labelwidth-\labelsep}
\def\@listvi{\leftmargin\leftmarginvi
 \labelwidth\leftmarginvi\advance\labelwidth-\labelsep}
\pagestyle{empty}       % added by T. Nguyen Oct-31-89

















